Sequential Neural Models with Stochastic Layers

How can we efficiently propagate uncertainty in a latent state representation with recurrent neural networks? This paper introduces stochastic recurrent neural networks which glue a deterministic recurrent neural network and a state space model together to form a stochastic and sequential neural generative model. The clear separation of deterministic and stochastic layers allows a structured variational inference network to track the factorization of the model's posterior distribution. By retaining both the nonlinear recursive structure of a recurrent neural network and averaging over the uncertainty in a latent path, like a state space model, we improve the state of the art results on the Blizzard and TIMIT speech modeling data sets by a large margin, while achieving comparable performances to competing methods on polyphonic music modeling.

==> midi.tex <==
%!TEX root = nips_2016.tex

\subsection{Polyphonic music modelling}
We now test the proposed model on the task of modelling sequences of polyphonic music, using the four data sets of MIDI songs introduced in \citep{boulanger2012modeling}. 
Each data set contains more than 7 hours of polyphonic music of varying complexity: folk  tunes (\textit{Nottingham} data set), the four-part chorales by J.S. Bach (\textit{JSB chorales}), orchestral  music (\textit{MuseData}) and classical  piano  music  (\textit{Piano-midi.de}). 
A time step is represented by a binary vector denoting which among 88 piano notes (from A0 to C8) are active. On average, 3.9 notes are playing at each time step.
The amount of data in the MIDI data sets is much smaller than in the Timit and Blizzard data sets, hence these experiments will allow us to understand if \nm can generalize well even for smaller tasks. Also, while in Section~\ref{sec:speech} we used \nm to model sequences of real valued numbers, now the data is discrete.

We use the same model architecture as in Section \ref{sec:speech}, except for the output Bernoulli variables used to model the active notes. 
We reduced the number of parameters in the model to 300 deterministic hidden units for the GRU networks, and 100 stochastic units whose distributions are parametrized with neural networks with 1 layer of 500 units. 
We report the results using smoothing and learning the residual between the mean of the predictive prior and the one of the variational approximation, but the performances using filtering and learning directly the mean of the variational approximation are now similar. 
We believe that this is due to the small amount of data and the fact that this modelling task is much simpler than the one in the previous section\todo{I'm not sure though. Any ideas?}.
Training of \nm on an NVIDIA Titan X GPU takes less than 15 minutes for the JSB chorales and Piano-midi.de data sets, and around 30 minutes for the Nottingham and MuseData data sets.

Table \ref{tab:result_midi} compares the average log-likelihood on the test sets obtained with \nm and the models introduced in \cite{gan2015deep,gu2015neural,Bayer2014,boulanger2012modeling}. 
As done in Section~\ref{sec:speech}, we prefer to report the more conservative estimate of the ELBO in Table \ref{tab:result_midi}, rather than approximating the log-likelihood with importance sampling as some of the other methods do. 
We see that \nm performs comparably to other state of the art methods in all four data sets\todo{RNN-NADE only works for discrete data?}. Also, the stochasticity in the model makes \nm very robust against overfitting.\todo{Make sure we address the  comments in the NIPS reviews of VRNN and TSBN paper:
https://media.nips.cc/nipsbooks/nipspapers/paper\_files/nips28/reviews/1686.html
https://media.nips.cc/nipsbooks/nipspapers/paper\_files/nips28/reviews/1461.html}


\begin{table}[t]
    \centering
    \begin{tabular}{c || c | c | c | c}
        \toprule
        \textbf{Models} & \textbf{Nottingham} & \textbf{JSB chorales}  & \textbf{MuseData} & \textbf{Piano-midi.de}  \\
\hline
\nm   & $\geq -2.94$   & $\geq -4.74$  & $\geq -6.28$ & $\geq -8.20$  \\
TSBN   & $\geq -3.67$   & $\geq -7.48$  & $\geq -6.81$  & $\geq -7.98$    \\
NASMC   & $\approx -2.72$   & $\approx \mathbf{-3.99}$  & $\approx -6.89$ & $\approx -7.61$     \\
STORN   & $\approx -2.85$  & $\approx -6.91$  & $\approx -6.16$  & $\approx -7.13$    \\
RNN-NADE   & $\approx \mathbf{-2.31}$  & $\approx -5.19$  & $\approx \mathbf{-5.60}$  & $\approx \mathbf{-7.05}$    \\
RNN   & $\approx -4.46$  & $\approx -8.71$  & $\approx -8.13$  & $\approx -8.37$  
   \\
    \end{tabular}
\caption{Average log-likelihood on the test sets. The TSBN results are from \cite{gan2015deep}, NASMC from \cite{gu2015neural}, STORN from \citep{Bayer2014}, RNN-NADE and RNN from \citep{boulanger2012modeling}.} \label{tab:result_midi}
\end{table}
